Testing Junta Truncation

We consider the basic statistical problem of detecting truncation of the uniform distribution on the Boolean hypercube by juntas. More concretely, we give upper and lower bounds on the problem of distinguishing between i.i.d. sample access to either (a) the uniform distribution over $\{0,1\}^n$, or (b) the uniform distribution over $\{0,1\}^n$ conditioned on the satisfying assignments of a $k$-junta $f: \{0,1\}^n\to\{0,1\}$. We show that (up to constant factors) $\min\{2^k + \log{n\choose k}, {2^{k/2}\log^{1/2}{n\choose k}}\}$ samples suffice for this task and also show that a $\log{n\choose k}$ dependence on sample complexity is unavoidable. Our results suggest that testing junta truncation requires learning the set of relevant variables of the junta.

==> scratch.tex <==

\newpage



\subsection{Reductions}\label{subsec:reductions}
We now prove our lower bound of $\log\binom{n}{k}$ on the sample complexity of any algorithm testing for truncation by $\mathcal{J}_{k,n}$. In our lower bound it will be convenient to define a weaker class of algorithms for testing truncation.
\begin{definition}
    Given a class $\mathcal{F}$ of $n$-bit Boolean functions, we say that an algorithm $\mathcal{A}$ \textit{weakly tests for truncation by $\mathcal{F}$} using $t$ samples if 
    \begin{align*}
        \frac1{2|\mathcal{F}|}\sum_{f\in\mathcal{F}}\Pr_{(\mathbf{x}^1,\dots,\mathbf{x}^t)\sim \mathcal{U}_{f^{-1}(1)}^t}[\mathcal{A}(\mathbf{x}^1,\dots,\mathbf{x}^t)=\mathcal{D}_{\mathcal{F},t}]+\frac12 \Pr_{(\mathbf{x}^1,\dots,\mathbf{x}^t)\sim \mathcal{U}_{n}^t}[\mathcal{A}(\mathbf{x}^1,\dots,\mathbf{x}^t)=\mathcal{U}_n^t]&\geq 0.99.
    \end{align*}
    Here $\mathcal{U}_{S}$ is the uniform distribution over $S\subseteq\{0,1\}^n$ and $\mathcal{U}_n=\mathcal{U}_{\{0,1\}^n}$.
\end{definition}
Note that algorithms weakly testing for truncation are an average case version of algorithms testing for truncation. That is, algorithms testing for truncation have a worst-case guarantee on error probability, while algorithms weakly testing for truncation only have an average-case guarantee on error probability. Thus we have the following fact.

\begin{fact}\label{fact:strong-to-weak}
    For any class of functions $\mathcal{F}$, an algorithm testing for truncation by $\mathcal{F}$ using $t$ samples is also an algorithm weakly testing for truncation by $\mathcal{F}$ using $t$ samples.
\end{fact}

Moreover, we use the following fact about algorithms testing for truncation. 

\begin{fact}\label{fact:subfamilies}
    Let $\mathcal{F}$ be a family of functions and let $\mathcal{G}\subseteq \mathcal{F}$. Any algorithm that tests for truncation by $\mathcal{F}$ using $t$ samples also tests for truncation by $\mathcal{G}$ using $t$ samples.
\end{fact}
\begin{proof}
    The algorithm $\mathcal{A}$ has error probability at most $\frac1{100}$ on sample sets drawn from $\mathcal{U}_{n}^t$ because it tests for truncation by $\mathcal{F}$. In a similar way, the $\mathcal{A}$ has error probability at most $\frac1{100}$ on sample sets drawn from $\mathcal{U}_{g^{-1}(1)}^t$ because it tests for truncation by $\mathcal{F}\supseteq \mathcal{G}$.
\end{proof}

Given these two facts, we see that in order to prove a lower bound on the sample complexity of testing for truncation by $\mathcal{J}_{k,n}$, it suffices to prove a lower bound on the sample complexity of weakly testing for truncation by some subclass of $\mathcal{J}_{k,n}$. We choose the subclass of parity functions $\chi_S$ for $S\subseteq[n]$ with $|S|=k$. The fact that this subclass forms a good error correcting code will be crucial in our analysis.

\subsection{Maximum Likelihood Estimation}
Fix a function class $\mathcal{F}$. Define the distribution $\mathcal{D}_{\mathcal{F},t}=\frac1{|\mathcal{F}|}\sum_{f\in \mathcal{F}}\mathcal{U}_{f^{-1}(1)}^t$. Let $\mathcal{D}$ be a random distribution that is $\mathcal{D}_{\mathcal{F},t}$ with probability $\frac12$ and $\mathcal{U}_n^t$ with probability $\frac12$.

Note that there exists an algorithm weakly testing for truncation by $\mathcal{F}$ using $t$ samples if and only if there is an algorithm $\mathcal{A}$ such that
\begin{align*}
    \Pr_{\mathcal{D},(\mathbf{x}^1,\dots,\mathbf{x}^t)\sim \mathcal{D}}[\mathcal{A}({\mathbf{x}}^1,\dots,\mathbf{x}^t)=\mathcal{D}]&\geq 0.99.
\end{align*}
Given this observation, it becomes more clear why we choose to prove lower bounds for weak testers. There is an optimal meta-algorithm for weak testing: maximum likelihood estimation. Given $t$ samples $(\mathbf{x}^1,\dots,\mathbf{x}^t)$, the maximum likelihood estimator makes the guess for the distribution $\mathcal{D}\in\{\mathcal{U}_n^t,\mathcal{D}_{\mathcal{F},t}\}$ that maximizes the likelihood $\Pr_{(\mathbf{y}^1,\dots,\mathbf{y}^t)\sim \mathcal{D}}[\vec{\mathbf{x}}=\vec{\mathbf{y}}]$.

The following lemma shows that proving lower bounds on the sample complexity of the maximum likelihood estimator suffices to prove lower bounds for the sample complexity of algorithms weakly testing for truncation. 

\begin{lemma}
If the maximum likelihood estimator, given $t$ samples, does not weakly test for truncation by $\mathcal{F}$, then there is no algorithm that given $t$ samples, weakly tests for truncation by $\mathcal{F}$. 
\end{lemma}
\begin{proof}
    Let $\mathcal{A}$ be any deterministic algorithm that given a sample set $(\mathbf x^1,\dots,\mathbf x^t)$ makes a guess as to whether the sample set was drawn from $\mathcal{U}_n^t$ or $\mathcal{D}_{\mathcal{F},t}$. Then the probability that $\mathcal{A}$ errs in the game described above is equal to
    \begin{align*}
        &\sum_{( y^1,\dots, y^t)\in\{0,1\}^n}\Pr_{\mathcal{D},(\mathbf x^1,\dots,\mathbf x^t)\sim \mathcal{D}}[\vec{\mathbf{x}}=\vec{ y},\mathcal{A}( y^1,\dots, y^t)\neq \mathcal{D}].
    \end{align*}
    For any $(y^1,\dots,y^t)\in(\{0,1\}^n)^t$ let $\overline{\mathcal{A}}(y^1,\dots,y^t)$ be the guess for the distribution not output by $\mathcal{A}$. For any individual $(y^1,\dots,y^t)$,
    \begin{align*}
        &\Pr_{\mathcal{D},(\mathbf x^1,\dots,\mathbf x^t)\sim \mathcal{D}}[\vec{\mathbf x}=\vec y,\mathcal{A}(\mathbf x^1,\dots,\mathbf x^t)\neq \mathcal{D}]\\
        =&\frac12\Pr_{(\mathbf x^1,\dots,\mathbf x^t)\sim \overline{\mathcal{A}}(y^1,\dots,y^t)}[\vec{\mathbf{x}}=\vec y]\\
        \geq & \frac12\Pr_{(\mathbf x^1,\dots,\mathbf x^t)\sim \overline{\mathrm{MLE}}(y^1,\dots,y^t)}[\vec{\mathbf{x}}=\vec y].
    \end{align*}
    % The last inequality follows because the MLE, given input sample set $(y^1,\dots,y^t)$, always outputs distribution $\mathcal{D}\in\{\mathcal{U}_n^t,\mathbcal{D}_{\mathcal{F},t}\}$ such that $\Pr_{(\mathbf x^1,\dots,\mathbf x^t)\sim \mathcal{D}}[\vec{\mathbf x}=\vec y]$ is larger than the other choice for $\mathcal{D}$. Note also that the second step crucially relies on the fact that $\mathcal{D}$ is selected uniformly from $\{\mathcal{U}_n^t,\mathcal{D}_{\mathcal{F},t}\}$.
\end{proof}

\subsection{The Lower Bound, Completed}\label{subsec:actual-lower-bound}






%%%% BACKUP LB
\section{Lower Bound}
\label{sec:lb}

In this section, we establish \Cref{thm:lb} by showing that any algorithm with the performance guarantee as in \Cref{thm:ub} must draw $\Omega(\log{n \choose k})$ samples from $\calD$. In more detail, we prove \Cref{thm:lb} by showing that it suffices to prove \emph{average case} lower bound against {maximum likelihood estimation (MLE)}, which we in turn establish this by showing that MLE requires $\log{n\choose k}$ samples to distinguish between $\calU_n$ and truncations of $\calU_n$ by an unknown \emph{parity} function on $k$ variables.

\subsection{Reducing to Maximum Likelihood Estimation}
\label{subsec:reduction-to-MLE}

\snote{I don't think we need to say anything about weak distinguishers?}

We first show that it suffices to show a lower bound against distinguishing algorithms with only an \emph{average case} guarantee. More formally, we consider the following class of algorithms:

\begin{definition} \label{def:weak-distinguisher}
    Let $\calM$ be the following mixture distribution over $\zo^n$:
    \[\calM = \begin{cases}
    \calU_n & \text{with probability}~1/2\\
    \calD \sim \calJ_n(k,\eps) & \text{with probability}~1/2
    \end{cases},\]
    where $\calD \sim \calJ_n(k,\eps)$ represents a uniform draw. 
    We say that an algorithm $\calA$ is a \emph{weak distinguisher} for junta truncation with $T$ samples if it has the following performance guarantee:
    \[\Prx_{\calD' \sim \calM}\sbra{\Prx_{\x{1},\dots,\x{T}\sim\calD'}\sbra{\calA(\x{1},\dots,\x{T}) ~\text{distinguishes correctly}}} \geq \frac{9}{10},\]
    where by ``distinguishes correctly'' we mean that if $\calD' = \calU_n$, then $\calA$ outputs ``un-truncated'' and if $\calD'\in\calJ_n(k,\eps)$, then $\calA$ outputs ``truncated''.
\end{definition}

Note that any algorithm with the performance guarantee as in \Cref{thm:ub} is trivially a weak distinguishers, and so it suffices for our purposes to prove a lower bound against weak distinguishers. 
Next, we define a weak distinguisher based on the maximum likelihood estimate.

\begin{definition} \label{def:mle-distinguisher}
    Given $T$ i.i.d. samples $(\x{1},\ldots,\x{T})$ drawn from some unknown distribution $D \in \{\calU_n\} \cup \calJ_n(k,\eps)$, we write $\MLE$ for the algorithm that outputs ``truncated'' (resp. ``un-truncated'') if $\calD' in \calJ_n(k,\eps)$ (resp. $\calD' =\calU_n$) maximizes the likelihood 
    \[\Prx_{\y{1},\ldots,\y{T}\sim\calD'}\sbra{(\y{1},\ldots, \y{T}) = (\x{1},\ldots,\x{T})}.\]
\end{definition}

The following fact is standard and follows immediately from \Cref{def:mle-distinguisher}.

\begin{fact} \label{fact:MLE-opt}
Given i.i.d. sample access to an unknown distribution $D \in \{\calU_n\} \cup \calJ_n(k,\eps)$, if $\MLE$ fails to weakly distinguish (cf.~\Cref{def:weak-distinguisher}) junta truncation with $T$ samples, then no algorithm weakly distinguishes junta truncation with $T$ samples. 
\end{fact}

% \begin{proof}
%     Let $\calA$ be any weak distinguisher for junta truncation. Note that the failure probability of $\calA$ is given by 
%     \begin{align*}
        
%     \end{align*}
    


%     Let $\mathcal{A}$ be any deterministic algorithm that given a sample set $(\mathbf x^1,\dots,\mathbf x^t)$ makes a guess as to whether the sample set was drawn from $\mathcal{U}_n^t$ or $\mathcal{D}_{\mathcal{F},t}$. Then the probability that $\mathcal{A}$ errs in the game described above is equal to
%     \begin{align*}
%         &\sum_{( y^1,\dots, y^t)\in\{0,1\}^n}\Pr_{\mathcal{D},(\mathbf x^1,\dots,\mathbf x^t)\sim \mathcal{D}}[\vec{\mathbf{x}}=\vec{ y},\mathcal{A}( y^1,\dots, y^t)\neq \mathcal{D}].
%     \end{align*}
%     For any $(y^1,\dots,y^t)\in(\{0,1\}^n)^t$ let $\overline{\mathcal{A}}(y^1,\dots,y^t)$ be the guess for the distribution not output by $\mathcal{A}$. For any individual $(y^1,\dots,y^t)$,
%     \begin{align*}
%         &\Pr_{\mathcal{D},(\mathbf x^1,\dots,\mathbf x^t)\sim \mathcal{D}}[\vec{\mathbf x}=\vec y,\mathcal{A}(\mathbf x^1,\dots,\mathbf x^t)\neq \mathcal{D}]\\
%         =&\frac12\Pr_{(\mathbf x^1,\dots,\mathbf x^t)\sim \overline{\mathcal{A}}(y^1,\dots,y^t)}[\vec{\mathbf{x}}=\vec y]\\
%         \geq & \frac12\Pr_{(\mathbf x^1,\dots,\mathbf x^t)\sim \overline{\mathrm{MLE}}(y^1,\dots,y^t)}[\vec{\mathbf{x}}=\vec y].
%     \end{align*}
%     % The last inequality follows because the MLE, given input sample set $(y^1,\dots,y^t)$, always outputs distribution $\mathcal{D}\in\{\mathcal{U}_n^t,\mathbcal{D}_{\mathcal{F},t}\}$ such that $\Pr_{(\mathbf x^1,\dots,\mathbf x^t)\sim \mathcal{D}}[\vec{\mathbf x}=\vec y]$ is larger than the other choice for $\mathcal{D}$. Note also that the second step crucially relies on the fact that $\mathcal{D}$ is selected uniformly from $\{\mathcal{U}_n^t,\mathcal{D}_{\mathcal{F},t}\}$.
% \end{proof}


\subsection{A Lower Bound Against $\MLE$}
\label{subsec:final-lb}

Throughout this section, it will be convenient for us to identify $\zo^n$ with $\F_2^n$ and to view Boolean functions $f\isazofunc$ as functions $f:\F_2^n\to\F_2$. 
Given a subset $S\sse[n]$, we write $\chi_S:\F_2^n\to\F_2$ for the (negated) \emph{parity} {function on $S$} defined by 
\[\chi_S(x) := 1 - \sum_{i\in S} x_i.\]
Let $\calP_n(k)$ be the collection of truncations of the uniform distribution over $\zo^n$ by parities on $k$ variables, i.e. 
\[\calP_n(k) := \cbra{\calU_n|_{\chi_S^{-1}(1)} \bigg|~ |S| = k}.\]



To establish this connection, let $\mathbf{V}$ be a random linear subspace of $\F_2^n$ sampled in the following way. Choose $\log\binom{n}{k}$ vectors uniformly randomly from $\F_2^n$. Then let $\mathbf{V}$ be the orthogonal complement of the span of the chosen vectors. Let $\mathbf{X}$ be the random variable defined as the number of weight-$k$ vectors in $\mathbf{V}$.

\begin{lemma}
    Given a sample set $(x^1,\dots,x^t)$ of $t=\log\binom{n}{k}$ many samples drawn from $\mathcal{U}_n^t$, the probability that the MLE guesses incorrectly that the samples came from $\mathrm{Trunc}_{\mathcal{P}_{n,k},t}$ is equal to the probability that $\mathbf{X}\geq 1$, where $\mathbf{X}$ is as defined previously.
\end{lemma}
\begin{proof}
    The probability that the MLE guesses incorrectly is equal to
    \begin{align*}
        &\Pr_{(x^1,\dots,x^t)\sim \mathcal{U}_n^t}[\Pr_{(y^1,\dots,t^t)\sim \mathrm{Trunc}_{\mathcal{P}_{n,k}}}[\vec x=\vec y]\geq \Pr_{(y^1,\dots,t^t)\sim \mathcal{U}_n^t}[\vec x=\vec y]]\\
        =&\Pr_{(x^1,\dots,x^t)\sim\mathcal{U}_n^t}[\Pr_{(y^1,\dots,t^t)\sim \mathrm{Trunc}_{\mathcal{P}_{n,k}}}[\vec x=\vec y]\geq \frac1{2^{nt}}]\\
        =&\Pr_{(x^1,\dots,x^t)\sim\mathcal{U}_n^t}[\frac{|\{S\subseteq[n]:|S|=k, \forall i\in[t] \sum_{j\in S}x^i_j=0\}|}{|\mathcal{P}_{n,k}|2^{(n-1)t}}\geq \frac1{2^{nt}}]\\
        =&\Pr_{(x^1,\dots,x^t)\sim\mathcal{U}_n^t}[|\{S\subseteq[n]:|S|=k, \forall i\in[t] \sum_{j\in S}x^i_j=0\}|\geq \frac{|\mathcal{P}_{n,k}|}{2^{t}}]\\
        =&\Pr_{(x^1,\dots,x^t)\sim\mathcal{U}_n^t}[|\{S\subseteq[n]:|S|=k, \forall i\in[t] \sum_{j\in S}x^i_j=0\}|\geq \frac{\binom{n}{k}}{\binom{n}{k}}]\\
        =&\Pr_{(x^1,\dots,x^t)\sim\mathcal{U}_n^t}[|\{S\subseteq[n]:|S|=k, \forall i\in[t] \sum_{j\in S}x^i_j=0\}|\geq 1].
    \end{align*}
    Note, however that this is exactly the probability that one samples $t=\log\binom{n}{k}$ uniformly random vectors $x^1,\dots,x^t$ from $\F_2^n$ and gets at least 1 weight-$k$ vector in the orthogonal complement of $\langle x^1,\dots,x^t \rangle$.
\end{proof}

\begin{lemma}\label{lem:second moment}
    The second moment $\mathbf X$ is bounded by
    \begin{align*}
        \E[\mathbf{X}^2]&\leq 3.
    \end{align*}
\end{lemma}
\begin{proof}
    Let $\mathbf{V}$ be the random linear subspace of $\F_2^n$ as before. Writing $\mathbf{X}=\sum_{x\in \F_2^n,|x|=k}\mathbf{1}_{x\in \mathbf V}$, we have that
    \begin{align*}
        \E[\mathbf{X}^2]&=\E[(\sum_{x\in \F_2^n,|x|=k}\mathbf{1}_{x\in \mathbf V})^2]\\
        &=\E[\sum_{x,y\in\F_2^n,|x|=|y|=k}\mathbf{1}_{x,y\in \mathbf V}]\\
        &=\sum_{x,y\in\F_2^n,|x|=|y|=k}\E[\mathbf{1}_{x,y\in \mathbf V}]\\
        &=\sum_{x,y\in\F_2^n,|x|=|y|=k}\Pr[x\in\mathbf V,y\in \mathbf V]\\
        &=\sum_{x\in\F_2^n,|x|=k}\Pr[x\in \mathbf V]+\sum_{x,y\in\F_2^n,|x|=|y|=k,x\neq y}\Pr[x\in\mathbf V,y\in \mathbf V].
    \end{align*}
    When $x\neq y$, we have that the events $x\in\mathbf V,y\in \mathbf V$ are independent. Therefore,
    \begin{align*}
        \E[\mathbf X]&=1+\sum_{x,y\in\F_2^n,|x|=|y|=k,x\neq y}\Pr[x\in\mathbf V]\Pr[y\in \mathbf V]\\
        &=1+\sum_{x,y\in\F_2^n,|x|=|y|=k,x\neq y}\frac1{2^{2t}}\\
        &=1+\sum_{x,y\in\F_2^n,|x|=|y|=k,x\neq y}\frac1{\binom{n}{k}^2}\\
        &\leq 1+2\\
        &=3\qedhere
    \end{align*}
\end{proof}

\begin{lemma}Let $\mathbf{X}$ be the random variable as before. Then
    \begin{align*}
        \Pr_{\mathbf{X}}[\mathbf{X}\geq 1]&\geq 0.01.
    \end{align*}
\end{lemma}
\begin{proof}
    We will prove by contradiction. Assume otherwise that $\Pr_{\mathbf{X}}[\mathbf{X}\geq 1]< 0.01$. First, note that by linearity of expectation,
    \begin{align*}
        \E[\mathbf X]&=\sum_{x\in\F_2^n, |x|=\binom{n}{k}}\Pr_{\mathbf{V}}[x\in \mathbf{V}]\\
        &=\sum_{x\in\F_2^n, |x|=\binom{n}{k}}\Pr_{x^1,\dots,x^t\sim \mathcal{U}_n}[\langle x^i,x\rangle=0\forall i\in[t]]\\
        &=\sum_{x\in\F_2^n, |x|=\binom{n}{k}}\prod_{ i\in[t]}\Pr_{x^i\sim \mathcal{U}_n}[\langle x^i,x\rangle=0]\\
        &=\sum_{x\in\F_2^n, |x|=\binom{n}{k}}\frac1{2^t}\\
        &=\frac{\binom{n}{k}}{\binom{n}{k}}\\
        &=1.
    \end{align*}
    Written another way, we have that
    \begin{align*}
        1&=\E[\mathbf X]=\sum_{i\geq 1}\Pr[\mathbf{X}\geq i].
    \end{align*}
    Rearranging, we have that
    \begin{align*}
        \Pr[\mathbf X\geq 1]&=1-\sum_{i\geq 2}\Pr[\mathbf X\geq i].
    \end{align*}
    Since we assumed that $ \Pr[\mathbf X\geq 1]<0.01$, we must have that $\sum_{i\geq 2}\Pr[\mathbf X\geq i]>0.99$.

    By \Cref{lem:second moment}, we have that $\mathrm{Var}(\mathbf X)=2$. Applying Chebyshev's inequality, we have that for $i\geq 2$,
    \begin{align*}
        \Pr[\mathbf{X}\geq i]&=\Pr[\mathbf{X}\geq \frac{i-1}{\sqrt2}\sqrt2]\\
        &\leq \frac1{(\frac{i-1}{\sqrt2})^2}\\
        &=\frac2{(i-1)^2}.
    \end{align*}
    Now, using that $\Pr[\mathbf{X}\geq i]\leq \Pr[\mathbf{X}\geq 1]<0.01$ for $i\geq 2$ as well, we have
    \begin{align*}
        \sum_{i\geq 2}\Pr[\mathbf{X}\geq i]&\leq \sum_{i\geq 2}\min(\frac2{(i-1)^2},0.01)\\
        &\leq \sum_{2\leq i\leq 15}0.01 + \sum_{i\geq 15}\frac{2}{(i-1)^2}\\
        &\leq 0.14+0.5\\
        &\leq 0.99.
    \end{align*}
    This contradicts that $\sum_{i\geq 2}\Pr[\mathbf X\geq i]>0.99$, so it must be that $\Pr[\mathbf{X}\geq 1]\geq 0.01$.
\end{proof}


